Scaling up Multi-domain Semantic Segmentation with Sentence Embeddings

We propose an approach to semantic segmentation that achieves state-of-the-art supervised performance when applied in a zero-shot setting. It thus achieves results equivalent to those of the supervised methods, on each of the major semantic segmentation datasets, without training on those datasets. This is achieved by replacing each class label with a vector-valued embedding of a short paragraph that describes the class. The generality and simplicity of this approach enables merging multiple datasets from different domains, each with varying class labels and semantics. The resulting merged semantic segmentation dataset of over 2 Million images enables training a model that achieves performance equal to that of state-of-the-art supervised methods on 7 benchmark datasets, despite not using any images therefrom. By fine-tuning the model on standard semantic segmentation datasets, we also achieve a significant improvement over the state-of-the-art supervised segmentation on NYUD-V2 and PASCAL-context at 60% and 65% mIoU, respectively. Based on the closeness of language embeddings, our method can even segment unseen labels. Extensive experiments demonstrate strong generalization to unseen image domains and unseen labels, and that the method enables impressive performance improvements in downstream applications, including depth estimation and instance segmentation.

==> data_statement.tex <==
Data Availability Statement

All data used in our are available from public repositories.

1. The datasets generated during and/or analysed during the current study are available in the public repository, indlucing:
1) http://mi.eng.cam.ac.uk/research/projects/VideoRec/CamVid/;
2) http://host.robots.ox.ac.uk/pascal/VOC/;
3) https://www.cvlibs.net/datasets/kitti/;
4) https://wilddash.cc/;
5) https://youtube-vos.org/dataset/vis/;
6) https://cs.nyu.edu/~silberman/datasets/nyu_depth_v2.html;
7) https://diode-dataset.org/;
8) http://www.scan-net.org/ScanNet/;
9) http://sintel.is.tue.mpg.de/;
10) https://cocodataset.org/.


==> discussion.tex <==

\section{Discussions} \label{sec:discussion}


{\small\textbf{Differences from fixed-point quantization approaches.}}
Our GroupNet is different from fixed-point quantization approaches~\cite{zhang2018lq, zhuang2018towards, zhou2016dorefa, mishra2018apprentice} in both the quantization algorithm and its underlying inference implementation. 

Note that in conventional fixed-point methods, the inner product between fixed-point weights and activations can be computed by bitwise operations.
Let ${\bw} \in {\mathbb{R}^M}$ and $\ba \in {\mathbb{R}^M}$
be the weights and activations, respectively.  they can be encoded by a linear combination of binary bases, respectively. 
In particular, $\bw$ and $\ba$ can be encoded by ${\bf{b}}_i^w \in {\{ - 1,1\} ^M}$ and ${\bf{b}}_i^a \in {\{ - 1,1\} ^M}$, where $i = 1,...,P$, respectively. Let $Q_P(\cdot)$ be any quantization function, and for simplicity, we here consider uniform quantization only. Then, the inner product of $\bw$ and $\ba$ can be approximated by
\begin{equation} \label{eq:fixed-point}
{Q_P}({{\bf{w}}^\mathrm{T}}){Q_P}({\bf{a}}) = \sum\limits_{i = 0}^{P-1} {\sum\limits_{j = 0}^{P-1} {{2^{i + j}}} } ({\bf{b}}_i^w \xor {\bf{b}}_j^a).
\end{equation}
where $\xor$ indicates the binary inner product, which can be efficiently implemented by
$\rm popcount$ and $\rm xnor$ bit-wise instructions that are commonly equipped in modern computers. According to Eq. (\ref{eq:fixed-point}), the computational complexity is $O(MP^2)$ for the fixed-point inner product.
Bearing the group-wise binary decomposition in Section \ref{sec:decomposition} in mind, it can be easily realized that the proposed GroupNet with $K$ bases has the same computational complexity with the conventional $P$-bit fixed point quantization when $K = 2^P$. However, compared with the $P$-bit fixed point quantization, the proposed GroupNet with $2^P$ bases introduces extra additions from the fusion of decomposition branches. It is worth noting that the convolution is implemented with two steps: $\rm im2col$ and $\rm GEMM$. The high-precision additions can be efficiently merged into the $\rm im2col$ operation of the succeeding layer during implementation. For $\rm im2col$ operation, most of the time is spend on data rearrangement, an extra tensor addition will have a very limited influence on its execution time.
Moreover, the extra additions only account for a small portion of the overall network complexity, which intrinsically limits the impact on the overall speed.
To justify our analysis, we provide speedup evaluations in Section \ref{sec:speed_benchmarks}. We also provide the analysis of the runtime training and inference memory cost in Section \ref{exp:runtime_memory}.


To emphasize, 
the proposed GroupNet enables much more flexible design of the quantization algorithm. 
Benefiting from the group-wise binary decomposition, the proposed GroupNet allows more fine-grained exploration space, where the quantization levels can be chosen from the continuous positive integer domain. In contrast, conventional fixed-point quantization requires the quantization levels to be the power of 2. For example, the bit-width of GroupNet with 5 bases is between 2-bit and 3-bit. Thus, GroupNet enjoys a flexible trade-off between complexity and accuracy by setting appropriate $K$.
Moreover, as introduced in Section \ref{sec:segmentation} and Section \ref{sec:detection}, 
our GroupNet is demonstrated to be more efficient in exploiting task-specific information or structures to compensate the quantization information loss.

Moreover, we define the model size of the full-precision model as $\Omega$. Then, the model size for GroupNet with $K$ bases becomes $K\Omega/32$ and the one for $P$-bit fixed-point quantization is $P\Omega/32$.

Based on the above analysis, we summarize that the proposed GroupNet
introduces small additional run-time cost caused by the extra addition operations, however, provides benefits in algorithm flexibility and performance.


\noindent\textbf{\kui{Differences between GroupNet
and 
other multiple binarizations methods.}}
In \cite{lin2017towards}, a linear combination of binary weight/activations bases are obtained from the full-precision weights or activations without being directly learned. In contrast, we directly design the binary network structure, where binary weights are end-to-end optimized. ~\cite{fromm2018heterogeneous, tang2017train, guo2017network, li2017performance} propose to recursively approximate the residual error and obtain a series of binary maps corresponding to different quantization scales.
However, it is a sequential process which cannot be paralleled. Also, all previous multiple binarizations methods belong to local tensor approximation. 
In contrast to value approximation, we propose a group decomposition approach to approximate the full-precision network. Moreover, tensor-based methods are tightly designed to local value approximation and may be hardly generalized to other tasks accordingly. In addition, our group decomposition strategy achieves much better performance than tensor-level approximation as shown in Section~\ref{sec:group_space}.

   


==> review1.tex <==
Reviewer #1: I found the idea of merging multiple datasets by replacing labels with sentence embeddings interesting. The proposed method is simple yet effective. The authors also conducted experiments on different datasets and tasks to illustrate their method's effectiveness.

Overall, this manuscript is well-written and easy to read. I suggest the following comments.

Major comments:
-       The illustrations in L34 of page 3 are not sufficient. The authors should have more explanations about the meaning of the different zero-shot segmentation settings to help the readers better understand.

\textbf{
More zero-shot settings...{meaning for each settings}}

-       The training efficiency section requires a more elaborated explanation. In Section 2 of the supplementary, the authors mentioned that they trained on 80 A100 GPUs for 5 days to get the best model. This computational cost is too heavy for most researchers. If there are any ways to reduce it, the authors can discuss them.

\textbf{This is mainly due to a large number of images, such as training ChatGPT or CLIP. We aim at exploring the boundary of the segmentation with all the annotated training data humans ever have.}


\textbf{Distillation/better initialization, optimization...}



-  The discussions of some optional steps are missing. This paper mentioned multi-scale testing in L31 on page 8 and distillation in Figure 4. The authors should have more discussions on their impact.

\textbf{Add Distillation ablation study. Add multi-scale testing settings.}



- In L50 of page 5, the authors set an adaptive threshold to the highest 30\% loss to select high-confident samples adaptively. How is this percentage determined?


\textbf{We conduct ablation studies on a small range of images.}



Minor comments:
-       In Figure 4, can we use a pooling layer to replace the Conv/Pool module (blue part)? The impact of the Conv/Pool module on the final performance needs more explanation.

\textbf{Thanks. + new experiments.}


-       Citation error in L4 of page 2.





Reviewer #2: This paper proposes to scale up multi-domain semantic segmentation with sentence embedding. The authors propose to replace class labels with CLIP-based text embeddings of contextual sentences, thus unifying the class labels across multiple datasets. The authors utilize pixelwise contrastive loss to train models with high-quality segmentation labels and noisy extra data, and also optimize their models with knowledge distillation from the CLIP encoder. Experiments on multiple datasets are provided.

(1) The insignificant contributions make this paper look like a simple combination of existing techniques without providing insights.
      - The text-embeddings for class labels is a very straightforward application of prompt[1].
      
\textbf{The motivation is different. We want to improve the generalization ability and build a universal segmenter with less human effort. They introduce the text as input while we use the text embedding as output. There are several advantages:
1. flexible for various datasets.

2. Change based on user inputs. +figures.

3. Merge more data without human effort.
}


- The pixel-level contrastive loss (eq.3-5) is very simple and not novel.

- The knowledge distillation loss is a very common technique and nothing new from the authors.           
The main novelty here is not the technical details, but the exploration of this problem.



(2) The comparison is unfair and inappropriate. The authors used huge amounts of extra information compared to existing work, including OpenImages, Objects365, and CLIP, to achieve a mediocre improvement in accuracy. It is not surprising and again makes the reader doubt the significance of this work.

\textbf{Significance: Exploration of the generalization ability of the current segmentation model.

We have extra strengths:
1.
2.
3.
}


(3) Quantitative analysis of the proposed method is way insufficient. The authors present evaluation results on various datasets, yet very few method analysis is provided. As an IJCV submission, the reader expects the extensive analysis to demonstrate the proposed method's effectiveness as well as the modules' advantage over previous works.


\textbf{ modules' advantage: Not the main contribution.}

\textbf{ 
Distill in Table 5. Deal with the dirty data.}







(4) Minor
      - The abstract needs to be revised.
      - Citation is missing in the left half of page 2-line 3.
      - The leading of the left half of page6-line14~23 needs to be corrected.

\textbf{Fixed.
}



All in all, the authors try to exploit the power of large-scale data and pre-trained CLIP's to tackle multi-domain segmentation, which is a good attempt. However, the current form of this manuscript is unsatisfying, and I encourage the authors to significantly improve their method and paper.



[1] Image Segmentation Using Text and Image Prompts, CVPR22




Reviewer #3: The paper proposes to use CLIP embedding as the target for semantic segmentation instead of traditional cross entropy with one-hot labels. This enables strong transferring to data with unseen domains and class labels, when it is paired with training datasets from diverse domains. The paper also proposes loss functions that accommodate noisy annotations and object box level annotations so it can train on larger scale datasets. Experiments on several segmentation datasets shows it outperforms previous method MSeg and training on individual datasets.

Strengths:
1. The motivation is clear and sound. The benefit of training multiple datasets on semantic segmentation is clear, and I think the community should move towards language embedding for semantic labels, rather than manual categorization into 1-hot labels.

2. The solution is simple and quite easy to follow. Compared with MSeg, organizing and unifying the datasets using language embedding becomes easier too.

3. The experiments are done on many training and testing datasets, closely following the settings of MSeg. The results clearly demonstrate the effectiveness of the methods.

Weaknesses:
1. LSeg [1] is an important prior work that uses CLIP language embedding to enhance semantic segmentation but is neither mentioned nor compared to in the paper.


\textbf{Compare with Lseg.  Motivation difference.
}

2. The downstream evaluation on depth and instanceseg seems not related with the main method. It is more similar to LSeg based on Fig.9 which uses language embedding as inputs rather than targets. Can authors explain why these are considered "downstream applications" of the proposed method?


\textbf{
Extensions to other tasks....}


3. The math equations can be improved. Equations can be centered rather than left-aligned.  What is d_gt and d_pred in 4.1 "Evaluation metrics" paragraph? They seems not defined.


\textbf{+more Explaination. Fix}



[1] Language-driven Semantic Segmentation. ICLR 2022.

